Data Lakes: A Survey of Functions and Systems

Data lakes are becoming increasingly prevalent for big data management and data analytics. In contrast to traditional 'schema-on-write' approaches such as data warehouses, data lakes are repositories storing raw data in its original formats and providing a common access interface. Despite the strong interest raised from both academia and industry, there is a large body of ambiguity regarding the definition, functions and available technologies for data lakes. A complete, coherent picture of data lake challenges and solutions is still missing. This survey reviews the development, architectures, and systems of data lakes. We provide a comprehensive overview of research questions for designing and building data lakes. We classify the existing approaches and systems based on their provided functions for data lakes, which makes this survey a useful technical reference for designing, implementing and deploying data lakes. We hope that the thorough comparison of existing solutions and the discussion of open research challenges in this survey will motivate the future development of data lake research and practice.

==> DS.tex <==
\subsection{Data science and machine learning}
\label{ssec:ds}
In recent years, one of most important applications of data lakes, is data science and machine learning 
% An important application of data lakes is  data science
\cite{DBLP:journals/pvldb/Miller18}. 
% If a data lake is used for data science tasks, we refer to it as a \emph{data science lake}. 

A straightforward solution to building a data  lake for data science/machine learning, is to 
apply  open-source tools that support data preparation pipelines and ML-related tasks (e.g., model training). 
For instance,  the proposal in \cite{DBLP:conf/icde/MehmoodGCKBVTR19}
 uses Spark to build the logistic regression model for sentiment analysis 
and Python  libraries (e.g., Matplotlib) for visualization.
%sec 3.5
There is also an open-source tool \cite{makhija2020loch} specialized for visualization.% in data lakes.  
  As discussed in Sec.~\ref{ssec:dlcloud}, modern enterprise data lakes often host large-scale data on  cloud platforms instead of on-premise, 
which is also more feasible for ML/DL model training, deployment and pipeline optimization \cite{10.1145/3448016.3457546}.

A more sophisticated manner is to integrate the specific data science tasks into the design of data lake functions. 
First,   when profiling the datasets, a data lake   might need to extract information relevant to the data science tasks \cite{zhang2020finding, DBLP:conf/sigmod/BrackenburyLMEU18}, e.g., manage notebook variables, and scientific topics of the experimental data. 
KAYAK \cite{maccioni2018kayak} divides the process of   data preparation into atomic operations, then allows data scientists to optimize the whole pipeline of data preparation.
Juneau \cite{zhang2020finding} allows the training/validation data augmentation, linking data, features extraction, and data cleaning. 
For each data science task, the corresponding similarity measures can be assembled based on the basic similarity measures as discussed in Sec.~\ref{sssec:relDS}.
For example, for data augmentation it also tries to find tables that can bring  new data instances to improve the information gain. In this way,   the accuracy of classification models could be improved.
If we take it more generally, given a data  lake with massive datasets, it is important to efficiently discover relevant data for data analysis  \cite{DBLP:journals/pvldb/Miller18}. 
The related dataset discovery systems introduced in Sec.~\ref{sssec:relDS} and Sec.~\ref{ssec:qds} are contributing to this promising direction.



==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> newDirections.tex <==
\section{Applications of data lakes}
\label{sec:newdir}
In this section, 
we discuss how data lakes can be used in modern applications. In doing so, we refer to methods discussed in previous sections that could be used for specific applications. 


\input{DS}
% \input{cloud}
\input{stream}

==> stream.tex <==
\subsection{Stream data lakes}
\label{ssec:sdl}
With the recent advances of Industrial 4.0, smart cities, and  e-commerce  websites,
a large volume of stream data at high speed needs to be selectively stored  and analyzed in near real-time.
Data lakes can store raw data and support heterogeneous data structures and formats, 
which makes data lakes a prominent technology in these scenarios, even though the concept of data stream management is based exactly on the assumption that there is not enough storage to keep all of them. Therefore, a core challenge in bringing both ideas together in \emph{stream data lakes} will be to find an optimal storage mix of storing raw data in limited time windows, reducing them by data analytics on the fly, and selective storage of aggregated time series.

Pennekamp et al. \cite{DBLP:conf/icphys/PennekampGHMQHG19}  propose to use data lakes to store, integrate, and collectively analyze vast amounts of heterogeneous data streams generated from sensors and machines in the production environment. Built upon Apache Kafka\footnote{\url{https://kafka.apache.org/}} and Flink\footnote{\url{https://flink.apache.org/}}, it supports ingesting stream data into Hadoop, and other DBMSs with the support of Kubernetes\footnote{\url{https://kubernetes.io/}}. 
%To support both real-time and batch data streams,
%In the architecture  of \cite{DBLP:conf/eScience/SuriarachchiP16}, the batch data processing is implemented based on Hadoop MapReduce and Spark, while the stream processing is based on Storm and Spark.
%looks not implemented, just an assumption
In a smart city use case, Manning et al. \cite{DBLP:conf/icde/MehmoodGCKBVTR19} propose  to apply Apache Flume and Spark for ingesting and processing stream data.
In Sec. \ref{sssec:dln}, we have introduced 
DLN  \cite{10.14778/3457390.3457403}, which discovers related attributes from large streams. 
In \cite{10.14778/3457390.3457403} the data processing system is Microsoft Cosmos \cite{10.14778/3476311.3476390} and the data processing language is Scope.
To ingest, stage and analyze stream data, in \cite{liu2020big} the data lake architecture is built upon Hadoop, and it applies NiFi, Kafka, and Sqoop.

To build a stream data lake, besides applying the existing open-source data stream libraries (e.g., Kafka, Flume, Storm, and Spark), another challenge is how to apply existing stream techniques  (e.g., Lambda architecture) in a data lake setting. For instance, the architecture proposed in \cite{DBLP:journals/access/MunshiM18} replaces the maintenance tier in Fig.~\ref{fig:rw-high-view} with the three parts of a Lambda architecture. Its batch layer serves all the data stored in Hadoop in batches and precomputes batch views; the speed layer handles streams ingested by Flume in real-time and computes real-time views; the serving layer integrates the batch views and real-time views, respectively, such that results can be 
passed to 
%provide for the queries from 
the exploration layer of the system for data querying and analytics.

 
